EnD: Entangling and Disentangling deep representations for bias correction

Artificial neural networks perform state-of-the-art in an ever-growing number of tasks, and nowadays they are used to solve an incredibly large variety of tasks. There are problems, like the presence of biases in the training data, which question the generalization capability of these models. In this work we propose EnD, a regularization strategy whose aim is to prevent deep models from learning unwanted biases. In particular, we insert an "information bottleneck" at a certain point of the deep neural network, where we disentangle the information about the bias, still letting the useful information for the training task forward-propagating in the rest of the model. One big advantage of EnD is that we do not require additional training complexity (like decoders or extra layers in the model), since it is a regularizer directly applied on the trained model. Our experiments show that EnD effectively improves the generalization on unbiased test sets, and it can be effectively applied on real-case scenarios, like removing hidden biases in the COVID-19 detection from radiographic images.

==> 3_method_kdelta.tex <==
\section{Entangling and Disentangling deep representations}
\label{sec:method}
\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{img/structure.png}
    \caption{\enzo{temporaneo... da aggiungere ref nel lesto}}
    \label{fig:structure}
\end{figure*}
In this section, after introducing the notation, we present \enzo{ABS}, a new regularization term, whose aim is to hide some \emph{discriminatory features} for a given task. In particular, NDR will be applied at the output of a given sub-network $\Pi_1$, which will be the input for a sub-network $\Pi_2$ computing the output of the ANN model, as already described in Sec.~\ref{sec:introduction}. NDR is designed to promote uncorrelated feature vectors belonging to the same discriminatory class: in such a way, the discriminatory information will be hidden during training. Hence, during the training phase, the objective function we aim to minimize will be
\begin{equation}
    \label{eq:uprule}
    J = \eta L + \gamma R_l
\end{equation}
where $L$ is the loss function for the trained task and $R_l$ is the proposed NDR term applied at $l$-th output layer, i.e. the $\Pi_1$ output.  Clearly, $\eta$ and $\gamma$ are two positive hyper-parameters. 
%level $l$ for\textbf{we apply at the $l$-th layer (hence, $l$ is the output layer for $\Pi_1$)}.\\
Finally. we are going to investigate the actual contribution of $R_l$ during back-propagation in $\Pi_1$.

\subsection{Preliminaries}
In this section we introduce the notation we are going to use for the rest of this work. Let us assume we work with an a-cyclic, multi-layer artificial neural network composed of $L$ layers, where layer $l=0$ is the input layer and $l=L$ the output layer. Each of the $l$ layers is made of $K_l$ neurons (or filters for convolutional layers). Hence, the $k$-th neuron ($k\in [1, K_l]$) in the $l$-th layer has:
\begin{itemize}
    \item $y_{l, k}$ as its own output.
    \item $\mathbf{y}_{l-1}$ as input vector.
    \item $\mathbf{w}_{l, k}$ as the weights (from which we identify the $p$-th as $w_{l, k, p}$) and $b_{l, k}$ as the bias.
\end{itemize}
Each of the neurons has its own activation function $\varphi_{l, k}(\cdot )$ to be applied after some affine function $f_{l, k}(\cdot)$ which can be, for example, a convolution or a dot product. Hence, the output of a neuron can be expressed by
\begin{equation}
    \label{eq::defy}
    y_{l, k} = \varphi_{l, k}\left[ f_{l, k} \left(\mathbf{w}_{l, k}, b_{l, k}, \mathbf{y}_{l-1} \right) \right]
\end{equation}
Each layer, during the forward-propagation step, will output a tensor $\mathbf{y}_l \in \mathbb{R}^{N_l \times M}$, where
\begin{itemize}
    \item $M$ is the mini-batch size.
    \item $N_l$ is the output size of the layer for a single input pattern.
\end{itemize}

\subsection{Data correlations}
\label{sec:ddc}
Let us consider the $l$-th layer in the ANN model, representing the output layer of $\Pi_1$. Clearly, $\mathbf{y}_l$ is a representation of the input samples. If these data can be grouped in $B$ \emph{bias classes}, and we aim at classifying these in $T$ \emph{target classes}, our mission is to train our model to correctly classifying the data into the $T$ possible classes preventing the use of the bias features provided in the data. Towards this end, we insert, between $\Pi_1$ and $\Pi_2$, an information bottleneck: the information related to these biases will be used as little as possible for the target classification task. Towards this end, we propose a two stages approach:
\begin{itemize}
    \item normalize each feature vector $\mathbf{y}_l$: in such a way, the norm will be the same for all the representations; \marco{La normalizzazione mi sembra un dettaglio tecnico per il calcolo della correlazione, non metterei tutta questa enfasi con 2 step}
    \item {\bf disentangle feature vectors having the same biases.} %handle the feature vectors exploiting both bias classes and target classes information.
\end{itemize}
We define $\mathbf{y}_l$ as the outputs at layer $l$. \marco{$\mathbf{y}_l$ definito sopra, piuttosto definiamo qui la versione normalizzata}
%We would like to ask every element in $\mathbf{y}_l^c$ being un-correlated: to have a correlation measure,} 
We can build a \emph{similarity matrix} $G_{l} \in \mathbb{R}^{M \times M}$, where $M$ is the mini-batch size:
\begin{equation}
    \label{eq:Gram}
    G_{l} = \left(\tilde{\mathbf{y}}_{l}\right)' \cdot \tilde{\mathbf{y}}_{l}
\end{equation}
where $(\cdot)'$ indicates transposed matrix and $ \tilde{\mathbf{y}}_{l}$ indicates a per-representation normalization
\begin{equation}
    \tilde{\mathbf{y}}_{l,i} = \frac{\mathbf{y}_{l,i}}{\| \mathbf{y}_{l,i} \|_2} \forall i \in [1, M]
\end{equation}
Hence, every $g_{l, i, j}$ entry between two patterns $i,j$ in $G_{l}$ indicates their correlation:
\begin{equation}
    g_{l,i,j} = \left(\tilde{\mathbf{y}}_{l,i} \right)' \cdot \tilde{\mathbf{y}}_{l,j}
\end{equation}
$G_{l}$ is a special case of \emph{Gramian matrix} as any $g_{l,i,j} \in [-1;+1]$ and indicates the difference in the direction between any two $\mathbf{y}_{l,i}$ and $\mathbf{y}_{l,j}$:
\begin{equation}
    \beta_{l,i,j} = \arccos{g_{l,i,j}}
\end{equation}
$G_{l}$ has some properties:
\begin{itemize}
    \item is a symmetric, positive semi-definite matrix.
    \item all the elements in the main diagonal are exactly 1 by construction.
    \item if the subset of outputs $\tilde{\mathbf{y}}_{l}$ forms an orthonormal basis $\forall~l$ (or, in this context, 
    equivalently $G_{l}$ is full-rank), then $G_l = \mathbb{I}$ by definition.
\end{itemize}
Handling these relations, we are going to build our regularization strategy, which consists in two terms:
\begin{itemize}
    \item a \emph{disentangling} term, whose task is to try to de-correlate as much as possible all the patterns belonging to the same bias class $b$;
    \item an \emph{entangling} term, which attempts to force correlations between data from different bias classes but having the same target class $t$.
\end{itemize}

\subsection{The EnD regularizer}
\marco{Menzionare da qualche parte il regulaizer incluso nella loss function}
Our regularization term consists in an overall structure
\begin{equation}
    R = \alpha R_{\perp} + \beta R_{\parallel}
\end{equation}
We know for all $ \tilde{\mathbf{y}}_{l,i}$ we can extract some bias class vector $\mathbf{b}$ and target vector $\mathbf{t}$. We can extract the features belonging to the b-th bias class and to the t-th target class by applying
\begin{equation}
    \label{eq:selection}
     \tilde{\boldsymbol{y}}_{l,i}^{b, t} =  \tilde{\boldsymbol{y}}_{l,i} \cdot \boldsymbol{\delta}_{b, \boldsymbol{b}} \cdot \boldsymbol{\delta}_{t, \boldsymbol{t}}
\end{equation}
where 
\begin{equation}
    \boldsymbol{\delta}_{i, \boldsymbol{v}} = \delta_{i, v_j} \forall j\in\left [1, \|\boldsymbol{v}\|_0\right ]
\end{equation}
$\|\cdot\|_0$ is the $\ell_0$ norm and $\delta_{i,j}$ is the Kronecker delta.

\subsubsection{Disentangling term}
Given our possibility to select the patterns belonging specifically to a bias class $b$ and to a target class $t$ as in \eqref{eq:selection}, we can extract all the examples belonging to a given bias class by simply computing
\begin{equation}
    \label{eq:biasexamples}
    \tilde{\boldsymbol{y}}_{l,i}^{b} =  \tilde{\mathbf{y}}_{l,i} \cdot \boldsymbol{\delta}_{b, \boldsymbol{b}}
\end{equation}
\marco{La  Kronecker delta non \`e strettamente necessaria; si potrebbe semplicemente dire. Let us define  $\tilde{\boldsymbol{y}}_{l,i}^{b}$ be the subset of pattern from
bias class $b$ in a mini-batch ...}
From \eqref{eq:biasexamples} we can build a Gramian matrix including the examples which belong to the $b$-th bias class
\begin{equation}
    \label{eq:Grambias}
    G_{l}^{b} = \left(\tilde{\mathbf{y}}_{l}^b\right)' \cdot \tilde{\mathbf{y}}_{l}^b
\end{equation}
This can be reduced to rank $M^b$: it is a sub-matrix of \eqref{eq:Gram}, and it holds all the properties as described in Sec.~\ref{sec:ddc}. In our learning problem, we would like to make $G_{l}^b \rightarrow \mathbb{I}~\forall~b$: towards this end, we can penalize all the off-diagonal elements
\begin{equation}
    \label{eq::strongregu}
    R_{\perp} = \frac{1}{B}\sum_{B} \frac{1}{2 M^b}\sum_{i\neq j} \left| g_{l,i,j}^b \right|
\end{equation}

\subsubsection{Entangling term}
While with $R_{\perp}$ we attempt to discourage the model to learn biases, we like to drive the model into building strong correlations between patterns belonging to different bias classes but to the same target class $t$. With an approach orthogonal to the one used to derive \eqref{eq:Grambias}, let us compute the Gramian matrix for the patterns belong to the same target class $t$:
\begin{equation}
\label{eq:Gramtarget}
    G_{l}^{t} = \left(\tilde{\mathbf{y}}_{l}^t\right)' \cdot \tilde{\mathbf{y}}_{l}^t
\end{equation}
where
\begin{equation}
    \tilde{\boldsymbol{y}}_{l,i}^{t} =  \tilde{\mathbf{y}}_{l,i} \cdot \boldsymbol{\delta}_{t, \boldsymbol{t}}
\end{equation}
Let us focus on the vector $\boldsymbol{g}_{l,i}^t$, extracted from the $j$-th column of $G_{l}^{t}$\enzo{aggiungere che j deve avere t come target}: it expresses how the $j$-th pattern correlates to all the other patterns which will be grouped to the same $t$-th target class. We ask the model to correlate the $j$-th pattern to all the other patterns having the same target class $t$, but belonging to different bias classes $b$. Towards this end, we can express our term as
\begin{equation}
    R_{\parallel} = 1- \frac{1}{M\cdot(B-1)} \sum_{t=1}^T \sum_{i=1}^{M^t} \sum_{b=1}^B \sum_{j=1}^{M^b} \frac{ {g}_{l,i, j}^t \cdot \delta_{b, \boldsymbol{b}_{j}}}{ M^b }
\end{equation}
\marco{Non abbiamo definito $M^t$ ... anche se evidente va fatto, inseriemo una spiegazione dei termini che vengono sommati}
\begin{figure}
    \begin{subfigure}[t]{\columnwidth}
        
        \includegraphics[width=0.5\columnwidth]{img/feature_space_beforeEnD.png}
        \caption{~}
        \label{fig:beforeEnd}
    \end{subfigure}
    \begin{subfigure}[t]{\columnwidth}
            \includegraphics[width=0.5\columnwidth]{img/feature_space_afterEnD.png}
            \caption{~}
            \label{fig:afterEnd}
    \end{subfigure}
    \caption{\enzo{da ref nel testo e commentare}}
    \label{fig:orthoeffect}
\end{figure}


